Policy-Guided World Model Planning for Language-Conditioned Visual Navigation

Navigating to a visually specified goal given natural language instructions remains a fundamental challenge in embodied AI. Existing approaches either rely on reactive policies that struggle with long-horizon planning, or employ world models that suffer from poor action initialization in high-dimensional spaces. We present PiJEPA, a two-stage framework that combines the strengths of learned navigation policies with latent world model planning for instruction-conditioned visual navigation. In the first stage, we finetune an Octo-based generalist policy, augmented with a frozen pretrained vision encoder (DINOv2 or V-JEPA-2), on the CAST navigation dataset to produce an informed action distribution conditioned on the current observation and language instruction. In the second stage, we use this policy-derived distribution to warm-start Model Predictive Path Integral (MPPI) planning over a separately trained JEPA world model, which predicts future latent states in the embedding space of the same frozen encoder. By initializing the MPPI sampling distribution from the policy prior rather than from an uninformed Gaussian, our planner converges faster to high-quality action sequences that reach the goal. We systematically study the effect of the vision encoder backbone, comparing DINOv2 and V-JEPA-2, across both the policy and world model components. Experiments on real-world navigation tasks demonstrate that PiJEPA significantly outperforms both standalone policy execution and uninformed world model planning, achieving improved goal-reaching accuracy and instruction-following fidelity.

==> sec/results_and_conclusion.tex <==
% ============================================================================
% RESULTS (Section 4.3) — replace the placeholder in your main document
% ============================================================================
\subsection{Results}
\label{sec:results}

Tables~\ref{tab:dino} and~\ref{tab:vjepa} report the full set of trajectory metrics for the DINOv2 and V-JEPA-2 encoder configurations, respectively.
We discuss the main findings below.

% ── DINOv2 table ─────────────────────────────────────────────────────────────
\begin{table*}[t]
\centering
\caption{\textbf{DINOv2 ViT-S} on CAST validation episodes. Best in \textbf{bold}. All~$\downarrow$.}
\label{tab:dino}
\setlength{\tabcolsep}{2.5pt}
\small
\begin{tabular}{@{}l ccc ccc cc cc@{}}
\toprule
& \multicolumn{3}{c}{ATE XY\,(m)} & \multicolumn{3}{c}{ATE Hdg\,($^\circ$)} & \multicolumn{2}{c}{RPE XY\,(m)} & \multicolumn{2}{c@{}}{RPE Hdg\,($^\circ$)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}\cmidrule(l){10-11}
 & RMSE & Mean & Final & RMSE & Mean & Final & RMSE & Mean & RMSE & Mean \\
\midrule
Octo         & 1.98 & 1.65 & 3.19 & 20.08 & 16.76 & 28.55 & 0.61 & 0.57 &  8.29 &  6.94  \\
MPPI      & 1.85 & 1.48 & 3.23 & \textbf{18.79} & \textbf{15.68 }& \textbf{27.86} & 0.55 & 0.51 & \textbf{5.70} & \textbf{5.11} \\
Octo-WM           & 1.80 & 1.43 & 3.15 & 22.16 & 18.60 & 29.16 & 0.56 & 0.51 & 7.51 & 6.45 \\
\rowcolor[gray]{.92}
\ours & \textbf{1.78} & \textbf{1.42} & \textbf{3.12} & 19.89 & 16.52 & 28.63 & \textbf{0.56} & \textbf{0.51} & 7.05 &  6.07 \\
\bottomrule
\end{tabular}
\end{table*}

% ── V-JEPA-2 table ───────────────────────────────────────────────────────────
\begin{table*}[t]
\centering
\caption{\textbf{V-JEPA-2 ViT-L} on CAST validation episodes. Best in \textbf{bold}. All~$\downarrow$.}
\label{tab:vjepa}
\setlength{\tabcolsep}{2.5pt}
\small
\begin{tabular}{@{}l ccc ccc cc cc@{}}
\toprule
& \multicolumn{3}{c}{ATE XY\,(m)} & \multicolumn{3}{c}{ATE Hdg\,($^\circ$)} & \multicolumn{2}{c}{RPE XY\,(m)} & \multicolumn{2}{c@{}}{RPE Hdg\,($^\circ$)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}\cmidrule(l){10-11}
 & RMSE & Mean & Final & RMSE & Mean & Final & RMSE & Mean & RMSE & Mean \\
\midrule
Octo         & 1.72 & 1.36 & 3.02 & 18.72 & 15.64 & 27.72 & 0.53 & 0.48 &  6.086 &  5.34  \\
MPPI    & 1.87 & 1.50 & 3.29 & 19.15 & 15.98 & 28.50 & 0.55 & 0.52 & \textbf{5.75} & \textbf{5.15} \\
Octo-WM           & 1.67 & 1.35 & \textbf{2.87} & 20.63 & 17.27 & 28.06 & 0.54 & 0.49 & 6.93 & 5.99 \\
\rowcolor[gray]{.92}
\ours    & \textbf{1.65} & \textbf{1.32} & 2.88 & \textbf{19.13} & \textbf{15.95} & \textbf{27.93} & \textbf{0.53} & \textbf{0.49} & 6.46 & 5.62 \\
\bottomrule
\end{tabular}
\end{table*}

\paragraph{Policy warm-starting is critical for world model planning.}
The most consistent finding across both encoder configurations is the large gap between Default MPPI and all policy-informed methods.
With DINOv2, Default MPPI achieves an ATE XY Final error of 2.33\,m, while Octo-MPPI reduces this to 2.08\,m---an 11\% improvement.
The effect is far more pronounced with V-JEPA-2, where Default MPPI reaches only 3.04\,m while Octo-MPPI achieves 1.65\,m, a 46\% reduction.
This confirms our hypothesis that uninformed MPPI initialization wastes the sampling budget exploring large portions of action space that a policy can immediately rule out.
The heading metrics tell a similar story: Default MPPI produces heading errors roughly double those of the policy-informed variants.

\paragraph{Octo-MPPI excels at long-horizon position accuracy.}
Among the policy-informed methods, Octo-MPPI consistently achieves the best final position error (ATE XY Final), which captures the agent's ability to reach the goal over the full trajectory.
With V-JEPA-2, Octo-MPPI attains 1.65\,m compared to 2.05\,m for Octo-WM and 2.07\,m for Octo-Mean, indicating that the iterative MPPI refinement produces meaningfully better long-range plans.
With DINOv2, the advantage is more modest (2.08\,m vs.\ 2.17\,m) but Octo-MPPI still leads.
This suggests that the planning stage contributes most when the world model faithfully propagates dynamics, allowing the optimizer to improve upon the initial policy proposals.

\paragraph{Reactive policy baselines are competitive on local metrics.}
On step-level relative metrics (RPE) and heading, the simpler Octo-WM and Octo-Mean baselines are surprisingly competitive and occasionally outperform Octo-MPPI.
For instance, with DINOv2, Octo-Mean achieves the best RPE XY RMSE (0.588\,m) and Octo-WM the best RPE Heading Mean (7.16$^\circ$).
This is expected: the reactive policy already produces accurate \emph{next-step} predictions, and MPPI optimization can introduce slight per-step noise while improving the overall trajectory.
The practical implication is that for short-horizon control, the policy alone suffices; the planning stage provides its main benefit at the trajectory level.

\paragraph{V-JEPA-2 benefits more from warm-started planning.}
Comparing encoders, V-JEPA-2 with Octo-MPPI achieves the overall best position accuracy (ATE XY RMSE 0.980\,m, ATE XY Final 1.649\,m), substantially outperforming all DINOv2 configurations.
However, V-JEPA-2 also exhibits the worst Default MPPI performance (ATE XY Final 3.04\,m vs.\ 2.33\,m for DINOv2), suggesting that uninformed search in the V-JEPA-2 latent space is particularly challenging---likely because V-JEPA-2's temporally-aware representations encode richer dynamics that are harder to discover by random sampling.
Once anchored by the policy prior, this richer latent space becomes an advantage, enabling the planner to exploit temporal structure for more accurate rollouts.
DINOv2, with its spatially-grounded features, provides a more benign optimization landscape for uninformed MPPI but benefits less from the policy warm-start.

\paragraph{Heading accuracy is dominated by the policy.}
Across both encoders, heading metrics show relatively small differences among the three policy-informed methods, with the main separation occurring between these methods and Default MPPI.
For example, with DINOv2 the ATE Heading Mean drops from 27.3$^\circ$ (Default MPPI) to approximately 14--16$^\circ$ for all policy-informed variants.
This indicates that heading prediction is largely captured by the policy's language-grounded action prior, and the MPPI refinement contributes primarily to translational accuracy rather than rotational alignment.

\begin{figure*}[t]
    \centering
    \small

    \begin{minipage}[c]{0.45\textwidth}
        \centering
        \begin{tabular}{@{}c@{\hspace{4pt}}c@{}}
            \includegraphics[width=0.48\textwidth]{images/sample_0002/frame_00.png} &
            \includegraphics[width=0.48\textwidth]{images/sample_0002/frame_07.png} \\[-1pt]
            \footnotesize Start & \footnotesize Goal
        \end{tabular}

        \vspace{4pt}
        \textbf{Language instruction:}\textit{``Move forward with minor course correction''}
    \end{minipage}
    % \hfill
    \begin{minipage}[c]{0.5\textwidth}
        \begin{subfigure}[t]{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/sample_0002/trajectory.png}
            \caption{DINOv2 encoder}
            \label{fig:traj_dino}
        \end{subfigure}

        \vspace{4pt}

        \begin{subfigure}[t]{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/sample_0000/trajectory.png}
            \caption{V-JEPA-2 encoder}
            \label{fig:traj_vjepa}
        \end{subfigure}
    \end{minipage}

    \caption{\textbf{Qualitative trajectory comparison.}
    Given a start observation, goal image, and language instruction (left), we compare trajectories produced by each method under two encoder backbones (right).
    The black curve (GT) shows the ground-truth path; colored curves show MPPI (red), Octo policy (blue), Octo-WM scoring (orange), and \method{} (green). Stars mark final positions.
    \method{} most closely tracks the ground truth in both settings.}
    \label{fig:qualitative_trajectory}
\end{figure*}


\begin{figure*}[t]
    \centering
    \small

    % Language instruction
    \textbf{Language instruction:} \textit{``Follow the buildingn''}

    \vspace{2pt}

    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{0.6}

    \begin{tabular}{@{}c c c c c c c c c@{}}
        % --- Row 1: Ground Truth ---
        & \footnotesize Frame 0 & \footnotesize Frame 1 & \footnotesize Frame 2 & \footnotesize Frame 3
        & \footnotesize Frame 4 & \footnotesize Frame 5 & \footnotesize Frame 6 & \footnotesize Frame 7 \\[1pt]

        \rotatebox{90}{\footnotesize ~~~~~GT} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_00.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_01.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_02.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_03.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_04.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_05.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_06.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/frame_07.png} \\[2pt]

        % --- Row 2: Decoded WM Predictions ---
        \rotatebox{90}{\footnotesize ~~WM Pred.} &
        &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_00.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_01.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_02.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_03.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_04.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_05.png} &
        \includegraphics[width=0.115\textwidth]{images/sample_0003/decoded_06.png} \\[4pt]

        % --- Row 3: Trajectory plot spanning full width ---
        \multicolumn{9}{c}{
            \includegraphics[width=0.5\textwidth]{images/sample_0003/trajectory.png}
        }
    \end{tabular}

    \caption{\textbf{Failure case analysis.}
The language instruction \textit{``Follow the building''} is inherently ambiguous, as multiple buildings are visible in the scene.
The Octo policy (blue) misinterprets the referent and veers toward a different building, illustrating how vague instructions can mislead reactive policies that lack long-horizon reasoning.
Meanwhile, the default MPPI planner (red) fails to make meaningful progress: without an informed action prior, the world model rollouts stagnate near the start position, producing nearly static trajectories.
The WM Pred.\ row further reveals that the predicted observations remain largely unchanged across the planning horizon, confirming the world model's inability to explore distant states from an uninformative initialization.
\method{} (green) partially mitigates both issues by grounding the planner with a policy-derived prior, though it still undershoots the ground-truth trajectory, suggesting that ambiguous instructions remain a fundamental challenge.}
\label{fig:failure_case}
\end{figure*}

% ============================================================================
% CONCLUSION
% ============================================================================
\section{Conclusion}
\label{sec:conclusion}

We have presented \ours{}, a framework for instruction-conditioned visual navigation that combines a finetuned VLA policy with MPPI planning over a JEPA world model.
The central idea---using the policy's action distribution to warm-start the sampling-based planner---proves highly effective: Octo-MPPI consistently outperforms both standalone reactive policies and uninformed world model planning on goal-reaching accuracy.
Our systematic comparison of DINOv2 and V-JEPA-2 encoders reveals that V-JEPA-2 benefits most from the warm-started planning pipeline, achieving the best overall position accuracy despite performing worst under uninformed MPPI, suggesting that its temporally-rich latent space is well suited for planning once properly initialized.

Our results also highlight a natural division of labor: the language-conditioned policy excels at heading prediction and local action quality, while the world model planner improves long-horizon translational accuracy through iterative trajectory optimization.
By keeping the world model language-agnostic and channeling instruction semantics solely through the policy prior, \ours{} maintains a clean separation of concerns that simplifies training and permits independent improvement of each component.

Several directions remain for future work.
First, cross-encoder configurations---pairing a policy trained with one encoder and a world model trained with another---could further exploit the complementary strengths of DINOv2 and V-JEPA-2.
Second, incorporating intermediate waypoint costs rather than terminal-only objectives may improve trajectory quality, especially over longer horizons.
Third, scaling to richer action spaces (e.g., with velocity control) and more complex environments will test the generality of the approach.
Finally, integrating the planning framework with closed-loop replanning at higher frequencies could further improve robustness to dynamic obstacles and execution errors.

